Near-IR observations of the young star [BHB2007]-1: A sub-stellar companion opening the gap in the disk

The presence of planets or sub-stellar objects still embedded in their native protoplanetary disks is indirectly suggested by disk sub-structures like gaps, cavities, and spirals. However, these companions are rarely detected. We present VLT/NACO high-contrast images in $J$, $H$, $K_S$, and $L^{\prime}$ band of the young star [BHB2007]-1 probing the inclined disk in scattered light and revealing the probable presence of a companion. The point source is detected in the $L^{\prime}$ band in spatial correspondence with complementary VLA observations. This object is constrained to have a mass in the range of 37-47 M$_{Jup}$ and is located at 50 au from the central star, inside the 70 au-large disk cavity recently imaged by ALMA, that is absent from our NACO data (down to 20 au). This mass range is compatible with the upper end derived from the size of the ALMA cavity. The NIR disk brightness is highly asymmetric around the minor axis, with the southern side 5.5 times brighter than the northern side. The constant amount of asymmetry across all wavelengths suggests that it is due to a shadow cast by a misaligned inner disk. The massive companion that we detect could, in principle, explain the possible disk misalignment, as well as the different cavity sizes inferred by the NACO and ALMA observations. The confirmation and characterization of the companion is entrusted to future observations.

==> ref_ans.tex <==
Reviewer #1:
The paper presents new infrared observations of a very young object with an edge-on disk and a large dust gap previously detected with ALMA. The NACO dataset reveals the disk in scattered light for the first time, and a substellar companion candidate inside the disk gap. The candidate is detected in the L' band, and its estimated mass could explain the observed gap. The work is well explained and justified, so I recommend publication in ApJ. Before acceptance, I would like the authors to address/discuss several points that can help to clarify some parts of the manuscript. I also include some minor points and suggestions at the end of the report.

Major points:
============

(1) Section 3.5, Substellar companion:

- According to Fig. 2, the companion candidate is embedded in the NIR circumstellar disk. Once the image is PSF-subtracted, how did the authors separate the disk emission from the companion candidate emission?

- If the L' emission is indeed related with a substellar companion with mass between 40-65 MJup, what would be the JHKs-magnitudes of this BD according to evolutionary models? Are these magnitudes consistent with the non-detection of the BD in the JHKs images? Please, explain this in the manuscript. 

- If the L' detection is indeed related with an embedded companion, could the L' emission come from a circumplanetary disk and not from the object itself? Please, discuss this possibility.

AUTHORS: The three points that the referee addressed above are connected, so we answer all of them here. The main text reads now: 


(2) Section 3.3: stellar parameters

There are some considerations that would be useful to mention/address in this section:

** Stellar luminosity estimation: I would mention that the object is surrounded by a highly inclined circumstellar, so its stellar
luminosity is probably underestimated. As a consequence, the source can look older when comparing its position in the HR diagram with PMS tracks (see e.g. Comerón et al. 2003). If the star is younger, this also affects the mass estimation of the companion candidate.

AUTHORS: We agree with the referee. Garufi et al. 2018 found in fact that stars with a very inclined disk look on average older than the other stars. This caveat has been added to the text.

** Discrepancy between the photometric and the dynamical mass of
[BHB2007]-1:

The authors have written that 'In the context of the PMS tracks, only a miscalculation of the Teff can reconcile the photometric and the dynamical mass'.

I think this conclusion deserves some discussion:

If the authors assume that the Teff is wrong, what would be the
expected Teff for a 2.2 Msun star at the age of BHB2007-1 according to PMS tracks? They will probably obtain a value of Teff >> 4000K, and a stellar luminosity inconsistent with the one they have derived.

Note that Covey et al. (2010) estimated the SpT of BHB2007-1 using spectral line indexes well suited for late-type stars. They were measured on good quality JHK spectra. In fact, the IR spectrum of this star shows lines and bands typical of K-type objects (see their Figure 6). Therefore, I do not find a good reason to believe that Covey's Teff estimation can be off by thousand degrees. 

AUTHORS: Indeed, an effective temperature of more than 5000 K would be necessary to reconcile the photometric and dynamical mass while such an offset appears implausible based on the spectra analyzed by Covey et al. The text has been changed accordingly following the referee's comment.

If I assume that the Teff is correct, an alternative scenario to
explain the 'mass discrepancy' would be to consider that the central object is an unresolved binary with nearly equal-mass components. I admit this is just a quick guess. Have the authors considered this possibility? Would it be possible to explain the system architecture with a triple system (binary + companion candidate) or can you reject it?

Of course, a proper modeling of the SED with a star+disk would be
needed to study the effect of the edge-on disk on the stellar
luminosity, and the binary hypothesis (assuming the distance is
correct). I understand that this is beyond the scope of this paper, but I think it is important to explain in this section that there are properties of the central object that are still unclear, and difficult to reconcile with the observations.

AUTHORS: We must say that there has been, prior to submission, a discussion among the co-authors about the possibility that the central star is in reality an unresolved binary with nearly equal-mass components. Therefore, we agree with the referee's suggestions and added a comment on this possibility in the draft. 

Minor points and suggestions:
=============================

- Introduction:
'Lately, it was even possible to catch planets in the ...'

In some of the cited papers there were not planets detected, so I would say instead:
'it was even possible to look for planets...'

AUTHORS: We modified the main text according to the suggestion.

- Section 3.1, presence of a jet in the Ks-band image:

** Looking at the image, it is not so evident that the Ks-band faint emission is coming from a jet. I would rephrase the text: 'In the Ks band a faint emission perpendicular to the disk plane is detected. If the feature is real, and not residual light from the spiders, it might be related with a jet'.

AUTHORS: We modified the main text according to the suggestion.

** Jet in NB1.64 filter image? Although the NB_1.64 observations are not optimal, have the authors checked if there is some emission at the position of the Ks band detection? Since this filter is centered at the [FeII] 1.64 micron line, a tracer of jets in young objects, it would be interesting to double-check.

AUTHORS: We thank the referee for the suggestion. Indeed we checked for emission in the image, but the poor quality of it makes even hard the detection of the disk. We added a phrase in the main text. 

** Note that Covey et al. 2010 presented IR (JHK) spectra of the
source and it shows BrG in emission (also intense Paschen Beta).
Please, correct this in the text.

AUTHORS: We thank the referee for pointing out the available spectrum. We updated the main text. 

** Figure 2, Ks-band panel: for clarity, label the emission coming from the possible jet

AUTHORS: We modified the caption of Fig. 2.

- Section 3.2: Astrometry and photometry

** GAIA EDR3 parallax of [BHB2007]-1: Recently, Rybizki et al. (2021) have developed a classifier ('fidelity' parameter) to identify spurious astrometric solutions in GAIA EDR3. I suggest the authors to check this parameter for [BHB2007]-1 an -2, since it can provide useful information about the quality of the GAIA astrometric solution for the two objects.

AUTHORS: We are grateful to the referee for this very nice suggestion. We checked the fidelity parameter and indeed, as we suspected, the Gaia measurement is most likely spurious. We included this point to the main text. 

** Astrometric measurements (Table 1):

-- Can the authors comment if they detect any orbital motion
between BHB2007-2 A and B when comparing the two epochs?

-- BHB2007-2 AB: can the authors clarify if they used the
coordinates of A (and not the average of AB) to derive the
astrometric measurements with respect to BHB2007-1?

-- With these data, can you confirm that BHB2007-1 and BHB2007-2, are co-moving? This can be relevant since you are adopting the same distance for the two objects.

AUTHORS: Initially we did not measure the position of BHB2007-2 B because it is very faint in the narrow band filter NB_1.64. To answer to the point of the referee we used another ad hoc routine to detect the faint PSF, the errorbars for the object are greater than the others. The main text, which should clarify the three points, reads now:
"On the other hand, [BHB2007]-2 A and B are a physically bound system as they show the same differences with respect to [BHB2007]-1, inside the errorbar. Note that one of the images used for this measurement is the narrow band filter NB\_1.64, which has a very poor quality, and [BHB2007]-2 B has a low SNR. It is then difficult to infer any orbital motion due to the great errorbars. This binary is not co-moving to [BHB2007]-2, they may have different proper motions if they are located at similar distance from us."

** For clarity, I would inthe position of clude a Table with the derived photometry (JHKL') for all the sources detected in the NACO images.

AUTHORS: We included a Table in the main text.

- Section 3.3, Stellar properties:

** Add (line 129): (Teff = 4060K and 3346K, for -1 and -2, respectively, with typical uncertainties of +-300K)

AUTHORS: We modified the main text accordingly. 

** Suggestion: The authors have retrieved WISE data (W1) for the 2 targets. Since Spitzer has a higher angular resolution, maybe it would be better to use the IRAC 3.6 mic data from Brooke et al. 2007. If there is no a big difference between the two datasets, you can ignore this comment.

AUTHORS: We checked for the differences in between the two datasets and they are comparable inside the errorbars. The analysis of the stellar parameters does not change. 

- Section 3.4: Disk

Can you clarify if the faint filament is only detected in the H-band image or is it also detected in the other bands?

AUTHORS: We clarified in the main text.

- Section 3.5:

Include the L' magnitude of the primary used to derive the brightness of the companion candidate.

AUTHORS: We included the value in the main text, and updated the value for the mass of the companion since we recalculated the value for L', from the W1 magnitude of the primary.

